An Adaptive Checkpointing Scheme for Peer-to-Peer Based Volunteer Computing Work Flows

Volunteer Computing, sometimes called Public Resource Computing, is an emerging computational model that is very suitable for work-pooled parallel processing. As more complex grid applications make use of work flows in their design and deployment it is reasonable to consider the impact of work flow deployment over a Volunteer Computing infrastructure. In this case, the inter work flow I/O can lead to a significant increase in I/O demands at the work pool server. A possible solution is the use of a Peer-to- Peer based parallel computing architecture to off-load this I/O demand to the workers; where the workers can fulfill some aspects of work flow coordination and I/O checking, etc. However, achieving robustness in such a large scale system is a challenging hurdle towards the decentralized execution of work flows and general parallel processes. To increase robustness, we propose and show the merits of using an adaptive checkpoint scheme that efficiently checkpoints the status of the parallel processes according to the estimation of relevant network and peer parameters. Our scheme uses statistical data observed during runtime to dynamically make checkpoint decisions in a completely de- centralized manner. The results of simulation show support for our proposed approach in terms of reduced required runtime.

==> Makefile <==
#
# basic makefile 
#

PAPER=ckpt_modeling
INPUTS=

# assumes that $(PAPER).tex and $(PAPER).bib exist
SRC=$(addprefix $(PAPER), .tex .bib)
INPUTSTEX=$(addsuffix .tex, $(INPUTS))

# figs - DO NOT put files that are not regnerable!
#
FIGS= gnutella_peer_failure_rate overnet_peer_failure_rate \
workflow workflowP2P timeline2
FIGFILES=$(addsuffix .fig, $(FIGS))
EPSFILES=$(addsuffix .eps, $(FIGS))
PSFILES=$(addsuffix .ps, $(FIGS))
# ensure that every eps has an associated .fig
# a command called ps2edit can convert ps and eps files to .fig files

# other deps
DEPS=$(SRC) $(EPSFILES) $(PSFILES) $(INPUTSTEX) 

#
# shouldn't be any need to change what is below
#

BIN=$(addprefix $(PAPER), .ps .pdf)
 
# stuff that is created but that can be removed
JUNK=$(addprefix $(PAPER), .log .aux .dvi) $(EPSFILES) $(PSFILES) $(addsuffix .aux, $(INPUTS))

$(PAPER).pdf : $(PAPER).ps
	ps2pdf -dEmbedAllFonts=true -dSubsetFonts=true -dEPSCrop=true $(PAPER).ps

$(PAPER).ps : $(PAPER).dvi
	dvips -Ppdf -t letter -Pdownload35 $(PAPER)

$(PAPER).dvi : $(DEPS) 
	latex $(PAPER) 
	latex $(PAPER) > /dev/null

checkbib : $(PAPER).dvi $(PAPER).bib
	bibtex $(PAPER)
	latex $(PAPER) > /dev/null
	latex $(PAPER) > /dev/null

%.eps : %.fig 
	fig2dev -L eps "$<"  > "$@" 

%.ps : %.fig
	fig2dev -L ps "$<" > "$@"

clean:
	- /bin/rm -f $(JUNK) *.bak *~ $(PAPER).bbl $(PAPER).blg

clobber: clean
	- /bin/rm $(BIN)
 

